LDPTrace: Locally Differentially Private Trajectory Synthesis

Trajectory data has the potential to greatly benefit a wide-range of real-world applications, such as tracking the spread of the disease through people's movement patterns and providing personalized location-based services based on travel preference. However, privay concerns and data protection regulations have limited the extent to which this data is shared and utilized. To overcome this challenge, local differential privacy provides a solution by allowing people to share a perturbed version of their data, ensuring privacy as only the data owners have access to the original information. Despite its potential, existing point-based perturbation mechanisms are not suitable for real-world scenarios due to poor utility, dependence on external knowledge, high computational overhead, and vulnerability to attacks. To address these limitations, we introduce LDPTrace, a novel locally differentially private trajectory synthesis framework. Our framework takes into account three crucial patterns inferred from users' trajectories in the local setting, allowing us to synthesize trajectories that closely resemble real ones with minimal computational cost. Additionally, we present a new method for selecting a proper grid granularity without compromising privacy. Our extensive experiments using real-world data, various utility metrics and attacks, demonstrate the efficacy and efficiency of LDPTrace.

==> 6_analysis.tex <==
\section{Theoretical Analysis}\label{sec:theoretical-analysis}

\subsection{Privacy Analysis}

\subsection{Error Analysis}\label{sec:analysis-error}

\subsection{Computational Cost}

\subsection{Communication Cost}



% \subsubsection{Taylor series approximation for ratio}



\subsubsection{Mean of Markov probability}
Consider the unbiased estimation of frequency for location $i$: $E(c_i) = nf_i$, $n$ is the time of report. The Markov transition probability of $P_{ij} = \frac{c_i}{\sum c_j}$. Using the mean of ratio:
\begin{equation}
E(P_{ij}) = E(\frac{c_i}{\sum c_j}) \approx \frac{E(c_i)}{\sum E(c_j)} = \frac{f_i}{\sum f_j}
\end{equation}

therefore, the estimated transition probability is unbiased.~\yuntao{can we say it is unbiased?}

\subsubsection{Variance of Markov probability}
The variance of OUE is $\operatorname{Var}(c_i) = \frac{4ne^\epsilon}{(e^\epsilon-1)^2}$, and the covariance of $\operatorname{Cov}(c_i, \sum c_j)$ is:

\begin{equation}
\begin{aligned}
\operatorname{Cov}(c_i, \sum c_j) 
&=  \operatorname{Cov}(c_i, c_{i}) + \operatorname{Cov}(c_i, \sum c_{j\i}) \\
& = \operatorname{Cov}(c_i, c_{i}) + 0 \\
&= \operatorname{Var}(c_i)
\end{aligned}
\end{equation}

and define $\operatorname{Var}(c_i) = \sigma$, thus $\operatorname{Var}(\sum c_j) = 8\sigma$.Remember $P_{ij} =\frac{c_i}{\sum c_j}$, and the variance is:


\begin{equation}
\begin{aligned}
\operatorname{Var}(P_{ij}) 
&=  (\frac{f_m}{|\Set{T}|})^2 [\frac{\sigma^2}{(f_m)^2} - \frac{2\sigma^2}{f_m |\Set{T}|} + \frac{8\sigma^2}{|\Set{T}|^2}] \\
& = (\frac{f_i}{\sum f_j})^2 [ (\frac{\sigma}{f_i} - \frac{2\sqrt{2}\sigma}{\sum f_j})^2 + O(\sigma^2)] \\
&\propto \sigma^2
\end{aligned}
\end{equation}

\subsubsection{Error of reported transition}
Suppose $m$ is the grid size, thus the overall error of Markov transition is:

\begin{equation}
\begin{aligned}
\operatorname{Var}(\sum \sum P_{ij}) 
&= 8m^2\sigma^2 \\
& \approx \frac{m^2 n e^\epsilon}{(e^\epsilon-1)^2} 
\end{aligned}
\end{equation}

To minimize this, we drive the differential equations:

\begin{equation}
\begin{aligned}
m^\star = c\frac{e^\epsilon - 1}{e^\epsilon + 1}
\end{aligned}
\end{equation}

\subsection{Selection of Optimal Grid Size}\label{sec:select-grid-size}

Before uploaded to the server, users' trajectories are first gridded into a sequence of cells. Therefore, it is important to choose the appropriate grid size $N$. As $N$ reflects the degree of the spatial discretization, it has a direct influence on the global distributions of the spatial locations. Thus we should select a global level metric that measures the distribution of location points to evaluate the effectiveness of the chosen $N$. In our analysis, we consider the range query task, which is one of the most popular and important location-based service that measures the global distributions of the dataset. In the following analysis, we use a region that covers $r$ portion of the total area to perform a count query. \todo{The output of the query is the number of location points that falls in that region.}

There are mainly two sources of errors in our proposed method. The first is \textbf{estimation error.} When users upload their trajectories, noise is added to each uploaded Markov transition to meet the LDP requirements. As discussed in Section ~\ref{sec:analysis-error}, the total standard deviation of estimated Markov probability is in the order of $\sqrt{\frac{ne^\epsilon}{(e^\epsilon-1)^2}}$. When performing the range query, the region shadows about $rN^2$ cells. As we only considers neighboring transitions to keep the continuity of trajectory, each cell covers \todo{9} Markov transitions (neighbourhood and the virtual end point). Moreover, because the Markov chain model is directed and has sequential orders, transitions start from each cell will not intersect. Besides, each Markov transition is an independent random variable and thus the total variation of the covered cells equals the sum of all involved Markov transitions. \todo{transition error -> count error} Therefore, the total standard deviation introduced by the perturbation in this query is in the order of $\sqrt{r}N\times\sqrt{\frac{ne^\epsilon}{(e^\epsilon-1)^2}}$, which is proportional to $N$. That is to say, when the query size is fixed, the more grids the area is partitioned into, the larger the estimation error is.

\todo{how to cite ICDE} The other source of error is \textbf{utility error}, which is caused by the non-uniformity of point distribution. When reconstructing trajectories from grids, we assume that the spatial points are uniformly distributed inside each cell. If the authentic distribution is not uniform and the query region covers only a partial of one cell, the count number of points in the intersected area will have errors. To quantify the error, we need to estimate number of cells that fall on the border of the query region. For the rectangle query that covers $rN^2$ cells, its circumference is in the order of $\sqrt{r}N$ cells, thus the total data points in the border cells are in the order of $\frac{m}{N^2}\times \sqrt{r}N=\frac{\sqrt{r}m}{N}$, where $m$ is the number of total spatial points.

In conclusion, the goal of optimization is:
\begin{equation}
    minimize\ \sqrt{r}N\times\sqrt{\frac{ne^{\epsilon'}}{(e^{\epsilon'}-1)^2}} + \frac{\sqrt{r}m}{N}
\end{equation}
In the above equation, $\epsilon'=\epsilon_2/L$, where $L$ is the estimated $k$ quantile of the length distribution and $\epsilon_2$ is the privacy budget. Because we can't obtain $L$ before the spatial descretization, it needs to be estimated in advance. Intuitively, there is positive correlation between $L$ and the average geographic length of trajectories because if the real travel distance of a trace is long, it should have more cells after descritization. In our analysis, we use sampling interval $\frac{1}{f}$ and average point number $l$ to estimate the average geographical length of a dataset. In real-world scenaries, $f$ can be collected from the type of GPS sensors and $l$ can be easily obtained from public knowledge or history data. Generally speaking, if the sampling interval and the average point number is large, the collected trajectory length will be longer. Therefore, the estimated $L$ is on the order of $\frac{l}{f}$. For $m$, the total number of location points, we use $n_ul$ to calculate it, where $n_u$ is the number of users. Finally, we can obtain the result of the optimization problem:
\begin{equation}
    N = a_0\cdot \sqrt[4]{\frac{n_ul(e^{\epsilon f/a_1 l} - 1)^2}{e^{\epsilon f/a_1 l}}}
\end{equation}
The parameter $a_0$ depends on the uniformity of the points distribution in the dataset. If the dataset is more uniformly distributed, the utility error tends to be smaller and $N$ should also be small, thus $a_0$ is relatively small. \todo{do we need a1?}
